Multi-Robot Path Planning in Complex Environments via Graph Embedding

We propose an approach to solve multi-agent path planning (MPP) problems for complex environments. Our method first designs a special pebble graph with a set of feasibility constraints, under which MPP problems have feasibility guarantee. We further propose an algorithm to greedily improve the optimality of planned MPP solutions via parallel pebble motions. As a second step, we develop a mesh optimization algorithm to embed our pebble graph into arbitrarily complex environments. We show that the feasibility constraints of a pebble graph can be converted into differentiable geometric constraints, such that our mesh optimizer can satisfy these constraints via constrained numerical optimization. We have evaluated the effectiveness and efficiency of our method using a set of environments with complex geometries, on which our method achieves an average of 99.0% free-space coverage and 30.3% robot density within hours of computation on a desktop machine.

==> deprecated.tex <==
\begin{align}
\label{eq:metric}
\resizebox{.42\textwidth}{!}{$\METRIC\triangleq w_{\#r}\METRIC_{\#r}+w_{\#rc}\METRIC_{\#rc}+w_{sd}\METRIC_{sd}+w_{g}\METRIC_{g},$}
\end{align}
where $w_{\bullet}$ is the user-provided weight of the metric term $\METRIC_{\bullet}$. Since our algorithm is greedy and can converge to a local minima, some of these terms are also used as heuristics to guide our algorithm at an early stage, other terms can be tuned by users to balance different requirements of applications. Our first term, $\METRIC_{\#r}$ is defined as:
\begin{align*}
\METRIC_{\#r}(\GRAPH)\triangleq |\POSS|,
\end{align*}
which is the number of vertices contained in $\GRAPH$. This term reflects the number of robots that $\GRAPH$ can hold, but MPP problems might not be feasible for all these robots because $\GRAPH$ might not be connected. However, $\METRIC_{\#r}$ guides our algorithm to find more valid cells at an early stage and then try to connect term. Our second term, $\METRIC_{\#rc}$, is the number of robots in the largest connected component of $\GRAPH$:
\begin{align*}
\METRIC_{\#rc}(\GRAPH)\triangleq 
\fmax{\footnotesize{\GRAPH'\subseteq\GRAPH\;\text{connected}}}
(\METRIC_{\#r}(\GRAPH')),
\end{align*}
which is the maximal number of robots for which MPP problems are feasible. Note that $\METRIC_{\#r,\#rc}$ are discrete, non-differentiable terms that are related to both the topology and geometry of $\DGRAPH$. To increase $\METRIC_{\#r,\#rc}$, we need to update the topology so that there are more triangles in $\DGRAPH$ and also update the shape of triangles so that they are valid and satisfy condition 2. Our third term is the agent packing density averaged over the valid cells:
\begin{align*}
\METRIC_{sd}(\GRAPH)\triangleq\frac{\pi r^2 \METRIC_{\#r}(\GRAPH)}{\sum_{\text{valid cell in } \DGRAPH}|\text{cell}|}.
\end{align*}
$\METRIC_{sd}$ is a heuristic guidance term that biases our algorithm towards denser robot packing, when only a subset the workspace is covered by the robot. Our last metric term $\METRIC_{g}$ is a differentiable and pure geometric term that is only related to $\DGRAPH$. This term is the used to guide our algorithm if none of the cells in $\DGRAPH$ are valid at an early stage, in which case $\METRIC_{\#r}=\METRIC_{\#rc}=\METRIC_{sd}=0$. To derive $\METRIC_{g}$, we analyze a regular triangle that contains 3 corner points as illustrated in \prettyref{fig:density}. To satisfy condition 2, this triangle have an area at least:
\begin{align*}
\text{A}^*\triangleq\frac{\sqrt{3}}{4}(2\sqrt{3}+4)^2 r^2,
\end{align*}
which is also a local minima of the cell area under condition 2. Therefore, we speculate that valid cells will have an area larger than $\text{A}^*$ and define:
\begin{align*}
\METRIC_{g}\triangleq\sum_{\text{cell}}\fmin{}(0,|\text{cell}|-\text{A}^*),
\end{align*}
so that each cell contributes a negative value to the metric if its area is too smaller.

\begin{algorithm}[ht]
\begin{small}
\caption{\label{alg:greedy} Optimize $\METRIC$ with respect to $\DGRAPH$.}
\begin{algorithmic}[1]
\State \TE{Input:} Initial $\DGRAPH$
\State Compute $\METRIC\gets\METRIC(\DGRAPH,\MAPPING(\DGRAPH))$
\State Set terminate ($\mathcal{T})$$\gets$True
\While{$\mathcal{T})$}
\State Set terminate ($\mathcal{T})$$\gets$False
\State Set $\mathcal{T}$$\gets$True if edges collapsed
\State Set $\mathcal{T}$$\gets$True if edges split
\State Set $\mathcal{T}$$\gets$True if edges flipped
\State Set $\mathcal{T}$$\gets$True if $\DGRAPH$ improved during vertex smoothing
\State Set $\mathcal{T}$$\gets$True if $\DGRAPH$ improved during local optimization
\State Set $\mathcal{T}$$\gets$True if $\DGRAPH$ improved during global optimization
\EndWhile
\State Set terminate ($\mathcal{T})$$\gets$True
\While{$\mathcal{T})$}
\State Set terminate ($\mathcal{T})$$\gets$False
\State Set $\mathcal{T}$$\gets$True if edges collapsed
\State Set $\mathcal{T}$$\gets$True if edges flipped
\State Set $\mathcal{T}$$\gets$True if $\DGRAPH$ improved during vertex smoothing
\State Set $\mathcal{T}$$\gets$True if $\DGRAPH$ improved during local optimization
\State Set $\mathcal{T}$$\gets$True if $\DGRAPH$ improved during global optimization
\EndWhile

\State Return $\MAPPING(\DGRAPH)$
\end{algorithmic}
\end{small}
\end{algorithm}


\begin{figure}[ht]
\centering
\includegraphics[width=0.75\linewidth]{figs/placeholder.png}
\caption{\small{\label{fig:baseline2} We compare our method with our previous work in the supplementary document. This method also deteriorates when there are many narrow passages.}}
\vspace{-10px}
\end{figure}
